On the efficient representation and execution of deep acoustic models

In this paper we present a simple and computationally efficient quantization scheme that enables us to reduce the resolution of the parameters of a neural network from 32-bit floating point values to 8-bit integer values. The proposed quantization scheme leads to significant memory savings and enables the use of optimized hardware instructions for integer arithmetic, thus significantly reducing the cost of inference. Finally, we propose a "quantization aware" training process that applies the proposed scheme during network training and find that it allows us to recover most of the loss in accuracy introduced by quantization. We validate the proposed techniques by applying them to a long short-term memory-based acoustic model on an open-ended large vocabulary speech recognition task.

==> am.tex <==
% !TEX root = deepq_main.tex

\subsection{LSTM Equations}
\input{lstm_equations}

\subsection{Parameter reduction}
\label{subsec:am_parameter_reduction}
In order to reduce memory consumption and computation, we compress the previously described acoustic model using projection layers that sit between the outputs of an LSTM layer and both the recurrent and non-recurrent inputs to same and subsequent layers~\cite{SakSeniorBeaufays14}. In our system, we introduce projection matrices of rank 100 for the first four layers, and a projection matrix of rank 200 for the fifth hidden layer, as we have noticed the weight matrices' ranks increases with depth.

Of crucial importance, however, is that when a significant rank reduction is applied, it is not sufficient to initialize the projection layer's weight matrix randomly for training with the CTC criterion. In section~\ref{sec:training} we explore a number of options for better, faster and more stable training convergence for our model. They range from adding a multiplicative factor that along with the global learning rate scales the gradient of the projection layers' weights during backpropagation, to exploying a clever initialization proposed in~\cite{prabhavalkar2016} that uses the larger `uncompressed' model without the projection layer and jointly factorize its recurrent and (non-recurrent) inter-layer weight matrices at each hidden layer using a form of singular value decomposition to determine a shared projection layer.

